Autonomous Option Invention for Continual Hierarchical Reinforcement Learning and Planning

Abstraction is key to scaling up reinforcement learning (RL). However, autonomously learning abstract state and action representations to enable transfer and generalization remains a challenging open problem. This paper presents a novel approach for inventing, representing, and utilizing options, which represent temporally extended behaviors, in continual RL settings. Our approach addresses streams of stochastic problems characterized by long horizons, sparse rewards, and unknown transition and reward functions. Our approach continually learns and maintains an interpretable state abstraction, and uses it to invent high-level options with abstract symbolic representations. These options meet three key desiderata: (1) composability for solving tasks effectively with lookahead planning, (2) reusability across problem instances for minimizing the need for relearning, and (3) mutual independence for reducing interference among options. Our main contributions are approaches for continually learning transferable, generalizable options with symbolic representations, and for integrating search techniques with RL to efficiently plan over these learned options to solve new problems. Empirical results demonstrate that the resulting approach effectively learns and transfers abstract knowledge across problem instances, achieving superior sample efficiency compared to state-of-the-art methods.

==> sections/figures/visualization.tex <==

\captionsetup{font=small,skip=8pt}
\setlength{\belowcaptionskip}{-12pt}
\begin{figure}[t!]
     \centering
     \begin{subfigure}[b]{0.12\textwidth}
            \includegraphics[scale=0.15]{final_images/taxi_concrete.png}
        \end{subfigure}
         \begin{subfigure}[b]{0.12\textwidth}
            \includegraphics[scale=0.15]{final_images/taxi1.png}
        \end{subfigure}
        \begin{subfigure}[b]{0.12\textwidth}
            \includegraphics[scale=0.15]{final_images/taxi2.png}
        \end{subfigure}
         
       \caption{\small
       Visualization of some abstract options learned by \alg{} 
       in Taxi World. Left: Initial state of taxi, passenger, and destination. Middle: Option to navigate to the pickup location. Right: Option to navigate to the destination with the passenger. An abstract state in the initiation sets (solid red lines) and termination sets (solid green lines) are highlighted. The colors represent a heatmap of Q-values of abstract states (blue $>$ green $>$ white $>$ red).
        }
     \label{fig:visualization}
\end{figure}


==> sections/reproducibility.tex <==
\section{Reproducibility checklist}

This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced. Yes.
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results. Yes.
    \item Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper. Yes.
\end{itemize}
Does this paper make theoretical contributions? 
Yes.

\begin{itemize}
\item All assumptions and restrictions are stated clearly and formally. Yes.
\item All novel claims are stated formally (e.g., in theorem statements). Yes.
\item Proofs of all novel claims are included. Yes.
\item Proof sketches or intuitions are given for complex and/or novel results. Yes.
\item Appropriate citations to theoretical tools used are given. Yes.
\item All theoretical claims are demonstrated empirically to hold. Yes.
\item All experimental code used to eliminate or disprove claims is included. Yes.
\end{itemize}
Does this paper rely on one or more datasets?
No.\\
Does this paper include computational experiments? 
Yes.

\begin{itemize}
\item Any code required for pre-processing data is included in the appendix.
Yes.
\item
All source code required for conducting and analyzing the experiments is included in a code appendix.
Yes. 
\item
All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. Yes.
\item
All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from Yes. 
\item
If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. 
Yes.
\item
This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. 
Yes. 
\item
This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. 
Yes.
\item
This paper states the number of algorithm runs used to compute each reported result. 
Yes.
\item
Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. 
Yes.
\item
The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). 
Yes.
\item
This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. Yes.
\item
This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. 
Yes.
\end{itemize}


==> todo.tex <==
- better related work
- More analysis on results of each domain why it performs better in some domains than others?
- adaptive params
- ijcai reviews
- ppo params

Which exact tasks?
hypersensitivity to parameters
Highlight four special locations
Situating within Lifelong learning papers and definition
Should we actually use an episode in reverse to update qvalues?













For CASATs:
https://pdf.sciencedirectassets.com/271506/1-s2.0-S0957417423X00244/1-s2.0-S0957417423019693/main.pdf?X-Amz-Security-Token=IQoJb3JpZ2luX2VjEGEaCXVzLWVhc3QtMSJHMEUCICX0Nf8d9OjZAR5i9aXVPXlxWcQap56SxTua6U5uMPd6AiEA4o1pvQT08O5XGXvth2Nu8ZxekZ6Z3%2Bz5q3YjXb3GUzYquwUIqv%2F%2F%2F%2F%2F%2F%2F%2F%2F%2FARAFGgwwNTkwMDM1NDY4NjUiDAKDtJjriefdk8f3%2BiqPBWLGXOZ7Z5ykfG8yxYZP%2B%2Bf6D%2B4f%2F0f%2F8gQE6gYPHNiubpTq5z%2FiZujcE72JkIE%2FBfLASDOOcVGe7uNTpQ9ksU3wNabf0UKFt1Dx%2Br3QTr9eLH3RZ8NojuBOA5tVh99eec8%2BGdG79OxENC%2BeqJg8Rjf7%2B4lDDJVGf6iJPJUKEyIUBOe0yOPLk7DOVakOUh4duRtrm0HirLcahp1KTfVW0lCANRsMo8NpHaa0I0UBttCE8B6bdQ1eRkl75PGE1lqEkPipyHvyYLkfSOiC089866P9MPkulchYkqqHUit38wm8OSdPOK2xcdHeXtRQTAgvZ3IYvDdu2BOfjtSve7jLt16wWN1LJWwtjjltNg%2BoBKU5%2FFDkAZDrdjC1sIrZoeYJfNNiZTVlAn8tB3mMhUG2z6zutiQHoK7Gwutn0wVHZzVEUnGp5GIQL7jNVJiKlgLr4WxlF%2Btflg3CbTlhBMhaIkWPU2EhnteDy82Ae6fhVV67aJTvGtgjd%2FX0imFQed%2BEtwnJm6hxHjNljX8JJMQXtzZNbzWjMB5rrKC5pLe23oc%2FB5rV1Z4XvoxphLrnuXqFnAdVasGzcaDazdJNV4%2Fy7AmfryN6Ef3M6ClJn2YuSuL3kTkmgSlD8dwYG11UVAY9TY57DKZdBUv0sJjob26Gf5%2BgTFPmWGlVwJFGig%2Fcmp3%2F705rKXIFlxibYpy4VfQnzD9ag4Qkk4QDH8vjk9Hqu4E8CgcIlHvXtgjt%2B1xaQPzTi51TrOKCK3zuGqgWsjkVCnXqJQCJMLwGjtcgstiMWY16hqZmwtm7KdNhWesj%2B5spRAxS64xcPnma88l3xGM%2B8WXM%2FiGXM5RD3Z9d2spJGXcikoC2%2ByemKI1B%2BbXilfkwnI6qsQY6sQGhddo962SY9yRyOP4A8SEaWfTmL6QiHUzQTq0TJSEHqOZ7Jp8YGwu6GRsvXSpnWojcrIx44zuka6pu7KdNKDUdvj9BXS8ZqVnfnJEkh1G4PP4wqxGqsO3WLYxIONouWXv0WAeh6KB0PA97BG6nXOlIr0srpZInEi6DfU%2BpUortdJSP9Wb%2FJXr4aR44%2BlOO0dtcQbDNxDb4s0h%2BN8LvE9C8GJFNvCHtKhceCyc5s9Cr5R0%3D&X-Amz-Algorithm=AWS4-HMAC-SHA256&X-Amz-Date=20240425T182422Z&X-Amz-SignedHeaders=host&X-Amz-Expires=300&X-Amz-Credential=ASIAQ3PHCVTY42Q2AFEM%2F20240425%2Fus-east-1%2Fs3%2Faws4_request&X-Amz-Signature=4d907cacb3a1b2dd423c1921dbe5c541213aa416effa4ad1e8b14c544545aff0&hash=66db0e87424b8f83f9eedb530cab273aef44e4bcb9296d222808c77d647bf84c&host=68042c943591013ac2b2430a89b270f6af2c76d8dfd086a07176afe7c76c2c61&pii=S0957417423019693&tid=spdf-f7ddb038-5e92-4ab2-8a49-271d718d72bc&sid=4c12acdd782bf24df77864e73cce93d2da07gxrqa&type=client&tsoh=d3d3LnNjaWVuY2VkaXJlY3QuY29t&ua=151459520456500b59&rr=87a05e9eab0ca71b&cc=us
